Strong Directional Asymmetry through Modal Hybridization in All-Dielectric Metasurfaces

Direction-dependent optical responses enable multifunctional metadevices but often require spatially varying meta-atoms or precisely aligned multilayer architectures. Here, we demonstrate a simple amorphous-silicon nanodisk array that exhibits broadband directional spectral asymmetry under unpolarized illumination, without requiring complex patterning or stacking. Coupling between localized Mie resonances and nonlocal guided mode resonances supported by the residual a-Si film produces hybrid resonances whose excitation and interference depend on the illumination direction. Upon reversal of the illumination direction, the reflection and absorption spectra are reshaped, while reciprocal transmission remains identical. At normal incidence, the measured absolute forward-backward reflectance difference reaches 24.2% at 616 nm, with a mean absolute difference of 8.3% across 500-850 nm. A locally optimized geometry yields a simulated absolute directional absorptance difference of 79.7% at 800 nm and a mean absolute difference of 17.4% over the same range. Angle-resolved measurements reveal additional spectral control through distinct dispersion sensitivity of resonances. We exploit these responses to encode patterns through local variations in nanodisk width, enabling spectral filtering and direction-dependent visibility. We further demonstrate a functional QR code that is readable in forward reflection and transmission but concealed in backward reflection. Fabricated in a single lithographic patterning step, this platform combines geometric simplicity with multiple optical readout channels for a vast range of applications including authentication, information encoding, direction-selective light harvesting.

==> preamble.tex <==
% Safe, compatible packages
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{graphicx}
\usepackage[version=4]{mhchem}
\usepackage{mathtools}
\usepackage{amsmath, amssymb}
\usepackage{physics}
\usepackage{xcolor}
\usepackage{adjustbox}
\usepackage{float}
\usepackage{booktabs}
\usepackage[font=small,labelfont=bf]{caption}
\usepackage{lipsum}
\usepackage{tabularx}
\usepackage{makecell}
% Fix Unicode errors (optional)
\usepackage{newunicodechar}
\newunicodechar{​}{} % invisible char
\DeclareUnicodeCharacter{2009}{\,}

% Custom commands
\newcommand{\RomanNumeralCaps}[1]{\MakeUppercase{\romannumeral #1}}




==> sections/comp.tex <==
\section*{Competing interests} \label{sec:comp}
The Authors declare no competing interests.
